VQDNA: Unleashing the Power of Vector Quantization for Multi-Species Genomic Sequence Modeling

Similar to natural language models, pre-trained genome language models are proposed to capture the underlying intricacies within genomes with unsupervised sequence modeling. They have become essential tools for researchers and practitioners in biology. However, the hand-crafted tokenization policies used in these models may not encode the most discriminative patterns from the limited vocabulary of genomic data. In this paper, we introduce VQDNA, a general-purpose framework that renovates genome tokenization from the perspective of genome vocabulary learning. By leveraging vector-quantized codebooks as learnable vocabulary, VQDNA can adaptively tokenize genomes into pattern-aware embeddings in an end-to-end manner. To further push its limits, we propose Hierarchical Residual Quantization (HRQ), where varying scales of codebooks are designed in a hierarchy to enrich the genome vocabulary in a coarse-to-fine manner. Extensive experiments on 32 genome datasets demonstrate VQDNA's superiority and favorable parameter efficiency compared to existing genome language models. Notably, empirical analysis of SARS-CoV-2 mutations reveals the fine-grained pattern awareness and biological significance of learned HRQ vocabulary, highlighting its untapped potential for broader applications in genomics.

==> tables/tab_app_semi.tex <==
\begin{table}[ht]
    \vspace{-1.25em}
    \setlength{\tabcolsep}{0.5mm}
    \centering
    \caption{Semi-supervised learning with GTR on genome tasks.}
    % \vspace{-0.5em}
    \label{tab:app_semi}
\resizebox{\linewidth}{!}{
    \begin{tabular}{l|cc|cc|cc}
    \toprule
Dataset        & \multicolumn{2}{c|}{H3 (EMP)} & \multicolumn{2}{c|}{Covid (CVC)} & \multicolumn{2}{c}{CPD (all)} \\
Labels         & 1\%           & 10\%          & 1\%             & 10\%           & 1\%           & 10\%          \\ \hline
PL             & 62.37         & 67.63         & 58.39           & 61.45          & 59.97         & 63.84         \\
FlexMatch      & 64.85         & 70.79         & 61.82           & 69.10          & 63.61         & 66.43         \\
\grow\bf{+GTR} & \bf{68.19}    & \bf{72.25}    & \bf{64.74}      & \bf{70.56}     & \bf{66.02}    & \bf{68.72}    \\
    \bottomrule
    \end{tabular}
    }
    \vspace{-1.0em}
\end{table}


==> tables/tab_app_tokenizer.tex <==
\begin{table}[ht]
    \vspace{-1.25em}
    \setlength{\tabcolsep}{0.5mm}
    \centering
    \caption{Analysis of various tokenizers.}
    % \vspace{-0.5em}
    \label{tab:app_tokenizer}
\resizebox{\linewidth}{!}{
    \begin{tabular}{ll|ccc}
    \toprule
Method    & Tokenizer & Usage & Lin.  & FT    \\ \hline
DNABERT   & 6-mer     & 47    & 23.54 & 55.50 \\
HyenaDNA  & one-hot   & 100   & 5.47  & 54.10 \\
DNABERT-2 & BPE       & 99    & 36.53 & 71.02 \\ \hline
VQDNA     & Word2Vec  & 100   & 39.25 & 70.48 \\
VQDNA     & VQVAE     & 100   & 44.76 & 73.16 \\
VQDNA     & HRQ       & 100   & 48.87 & 74.32 \\
    \bottomrule
    \end{tabular}
    }
    \vspace{-1.0em}
\end{table}


==> tables/tab_multi_species_data.tex <==
\begin{longtable}{lll}

	\toprule
	\textbf{Category} & \textbf{Species} & \textbf{Num. of Nucleotides (M)}  \\
	\midrule
	\endfirsthead
	\multicolumn{3}{l}{\textit{(Continued from previous page)}} \\
	\midrule
	\textbf{Category} & \textbf{Species} & \textbf{Num. of Nucleotides (M)} \\
	\midrule
	\endhead
	\midrule
	\multicolumn{3}{r}{\textit{(Continued on next page)}} \\
	\endfoot
	\endlastfoot

 	\multirow{10}{*}{\textbf{Fungi}} & Ceratobasidium & 655.37 \\
& Claviceps Maximensis & 329.79 \\
& Fusarium Annulatum & 449.98 \\
& Melampsora & 699.52 \\
& Metschnikowia & 109.36 \\
& Mucor Saturninus & 391.17 \\
& Penicillium Chermesinum & 275.81 \\
& Saccharomyces Cerevisiae & 121.54 \\
& Sporopachydermia Quercuum & 155.71 \\
& Tranzscheliella Williamsii & 184.77 \\
& Xylariales & 399.96 \\
	
	\midrule
	
	\multirow{2}{*}{\textbf{Protozoa}} &  Phytophthora Sojae & 792.65 \\
& Pythium Apiculatum & 450.99 \\
	
	\midrule
	
	\multirow{7}{*}{\textbf{Mammalian}} 
 & Bubalus Bubalis & 28768.00 \\
& Camelus Dromedarius & 19757.02 \\
& Human & 31372.10 \\
& Macaca Assamensis & 27593.76 \\
& Macaca Nigra & 28217.13 \\
& Mus Musculus & 26545.98 \\
& Peromyscus Californicus & 24677.56 \\
	
	\midrule

 & Anas Zonorhyncha & 11697.08 \\
\textbf{Other} & Coregonus Clupeaformis & 26824.02 \\
\textbf{Vertebrate} & Gnathonemus Longibarbis & 7314.74 \\
& Myxocyprinus Asiaticus & 23407.19 \\
& Rhipidura Dahli & 10112.96 \\
	
 \midrule

\multirow{20}{*}{\textbf{Bacteria}} & Aeromonas & 47.33 \\
& Agrobacterium & 97.22 \\
& Alcaligenaceae Bacterium & 20.88 \\
& Aliivibrio & 46.48 \\
& Alphaproteobacteria Bacterium & 14.22 \\
& Amycolatopsis Antarctica & 63.43 \\
& Anaerostipes Faecis & 32.00 \\
& Arthrobacter & 36.27 \\
& Atopobium & 28.63 \\
& Bacillus Bc15 & 57.34 \\
& Bacillus Bs3 2021  & 43.51 \\
& Bacterium & 7.54 \\
& Bacteroidetes Bacterium Qs & 8.99 \\
& Breoghania Corrubedonensis & 53.32 \\
& Caldicoprobacter Oshimai & 27.25 \\
& Candidatus Cryptobacteroides Excrementipullorum & 27.63 \\
& Candidatus Dadabacteria Bacterium Rbg Combo & 11.49 \\
& Candidatus Dwaynia Gallinarum & 16.82 \\
& Candidatus Falkowbacteria Bacterium & 13.88 \\
& Candidatus Geothermincola Secundus & 24.76 \\
& Candidatus Gottesmanbacteria Bacterium & 11.08 \\
& Candidatus Nomurabacteria Bacterium Full & 6.29 \\
& Candidatus Portnoybacteria Bacterium Big Fil Rev & 8.17 \\
& Candidatus Regiella Insecticola & 20.62 \\
& Candidatus Roizmanbacteria Bacterium Combo All & 11.13 \\
& Candidatus Rokubacteria Bacterium & 22.06 \\
& Candidatus Saccharibacteria Bacterium & 6.55 \\
& Candidatus Staskawiczbacteria Bacterium Full & 6.79 \\
& Christensenella & 18.75 \\
& Clostridiaceae Bacterium & 29.62 \\
& Clostridiales Bacterium & 16.59 \\
& Clostridium Cag 505 & 21.26 \\
& Clostridium Mcc328 & 36.43 \\
& Clostridium Nexile & 38.43 \\
& Clostridium Uba3521 & 25.99 \\
& Collinsella Urealyticum & 19.45 \\
& Coprobacillus Cateniformis & 38.38 \\
& Cyanobium & 40.33 \\
& Dehalococcoidia Bacterium & 17.59 \\
& Enterobacteriaceae Bacterium & 41.46 \\
& Evtepia Gabavorous & 24.94 \\
& Firmicutes Bacterium & 36.66 \\
& Fulvivirga & 65.24 \\
\textbf{Bacteria} & Jeongeupia Chitinilytica & 39.11 \\
& Legionella Endosymbiont Of Polyplax Serrata & 5.30 \\
& Listeria Ilorinensis & 30.31 \\
& Maribacter Cobaltidurans & 46.40 \\
& Marinomonas & 37.73 \\
& Mesorhizobium & 65.15 \\
& Methyloceanibacter Caenitepidi & 34.25 \\
& Microvirga & 68.63 \\
& Mycolicibacter Engbaekii & 45.21 \\
& Novosphingobium & 46.18 \\
& Omnitrophica Wor Bacterium Rbg & 12.52 \\
& Pantoea & 43.14 \\
& Paraburkholderia Edwinii & 82.99 \\
& Parerythrobacter Lutipelagi & 30.98 \\
& Paulownia Witches Phytoplasma & 8.92 \\
& Polaromonas Eurypsychrophila & 41.61 \\
& Prevotella Ag 487 50 53 & 29.63 \\
& Prevotella Uba3619 & 31.72 \\
& Prevotella Uba634 & 18.51 \\
& Prochlorococcus Ag-321-I09 & 3.29 \\
& Prochlorococcus Ag-363-B18 & 15.54 \\
& Prochlorococcus Ag-402-L19 & 11.17 \\
& Prochlorococcus Scb243 498N4 & 14.12 \\
& Providencia & 41.89 \\
& Pseudomonas 35 E 8 & 63.56 \\
& Pseudomonas Bigb0408 & 59.52 \\
& Pseudomonas P867 & 62.01 \\
& Pseudomonas Promysalinigenes & 50.47 \\
& Roseobacter & 44.14 \\
& Salinicola Peritrichatus & 46.19 \\
& Salmonella S096 02912 & 48.09 \\
& Salmonella Zj-F75 & 47.87 \\
& Sinorhizobium & 65.53 \\
& Sodalis Ligni & 63.85 \\
& Sphaerochaeta & 28.61 \\
& Sphingobacterium & 36.55 \\
& Sphingomonas Carotinifaciens & 37.53 \\
& Sphingomonas Mesophila & 22.91 \\
& Sporosarcina Jiandibaonis & 36.30 \\
& Sporosarcina Ureilytica & 34.37 \\
& Staphylococcus Gdq20D1P & 28.50 \\
& Staphylococcus M0911 & 24.38 \\
& Streptococcus & 22.18 \\
\textbf{Bacteria} & Streptomyces 8401 & 88.39 \\
& Streptomyces Di166 & 88.71 \\
& Streptomyces Durbertensis & 59.24 \\
& Streptomyces Neau-Yj-81 & 118.84 \\
& Streptomyces Rk74B & 87.36 \\
& Thermopetrobacter & 26.06 \\
& Uncultured Kushneria & 35.31 \\
& Uncultured Phascolarctobacterium & 17.95 \\
& Uncultured Proteus & 35.66 \\
& Verrucomicrobiales Bacterium & 3.15 \\
& Vibrio & 41.47 \\
& Victivallis Lenta & 55.45 \\
& Virgibacillus Salexigens & 44.18 \\
& Xanthomonadales Bacterium & 37.47 \\

\bottomrule
\caption{Details statistics of the multi-species genome dataset for pre-training.}
\label{tb:multi_species_details}
\end{longtable}

